An Empirical Evaluation of Using Large Language Models for Automated Unit Test Generation

Unit tests play a key role in ensuring the correctness of software. However, manually creating unit tests is a laborious task, motivating the need for automation. Large Language Models (LLMs) have recently been applied to this problem, utilizing additional training or few-shot learning on examples of existing tests. This paper presents a large-scale empirical evaluation on the effectiveness of LLMs for automated unit test generation without additional training or manual effort, providing the LLM with the signature and implementation of the function under test, along with usage examples extracted from documentation. We also attempt to repair failed generated tests by re-prompting the model with the failing test and error message. We implement our approach in TestPilot, a test generation tool for JavaScript that automatically generates unit tests for all API functions in an npm package. We evaluate TestPilot using OpenAI's gpt3.5-turbo LLM on 25 npm packages with a total of 1,684 API functions. The generated tests achieve a median statement coverage of 70.2% and branch coverage of 52.8%, significantly improving on Nessie, a recent feedback-directed JavaScript test generation technique, which achieves only 51.3% statement coverage and 25.6% branch coverage. We also find that 92.8% of TestPilot's generated tests have no more than 50% similarity with existing tests (as measured by normalized edit distance), with none of them being exact copies. Finally, we run TestPilot with two additional LLMs, OpenAI's older code-cushman-002 LLM and the open LLM StarCoder. Overall, we observed similar results with the former (68.2% median statement coverage), and somewhat worse results with the latter (54.0% median statement coverage), suggesting that the effectiveness of the approach is influenced by the size and training set of the LLM, but does not fundamentally depend on the specific model.

==> algorithm.tex <==



\begin{algorithm}[tb]
\caption{Function \textit{GenerateTests}}
\label{alg:testGen}
\begin{algorithmic}[1]
	\Require 
	  \begin{tabular}[t]{l}
	    $N$: package name\\
	    $S$: set of API signatures discovered for $N$ using dynamic analysis\\
	    $H$: map API signature $\rightarrow$ set of code snippets containing definitions/uses 
	  \end{tabular}
	  
	\Ensure 
	  \begin{tabular}[t]{l}
	    \TAssert: passing tests with assertions\\
	    \TNoAssert: passing tests without assertions\\
	    \TFail: failing tests\\ 
	 \end{tabular}
	 
	\State $t_{\mbox{\scriptsize \it init}}$ = 
	            \begin{tabular}[t]{l}
	                \code{let _package = require(}$N$\code{)}\\
	                \code{assert = require('assert');}\\
	                $\bullet$ \code{// extension point}
	            \end{tabular} \Comment{initial test}
	               
    
    \State $W \leftarrow \{ t_{\mbox{\scriptsize \it init}} \}$ \Comment{initialize worklist}
    \State $\TAttempted \leftarrow \emptyset$  \Comment{to avoid trying the same test repeatedly}
    

    \While{$|\TAssert|+|\TNoAssert|+|\TFail| <$ number of tests to generate}
      \State select test $t$ from $W$
      \State select extension point $E$ in $t$ 
      \State select signature $s$ from $S$  \Comment{select API signature} 
      \State $h \leftarrow \textit{GetSnippets}(s)$  \Comment{fetch usage examples} 
      \State $t' \leftarrow$ extend $t$ with ``\code{// test} $S$'' at $E$
      \State add $h$ to $t'$ \Comment{add available hints}
      
      \State \success $\leftarrow$ false
      \State \nrAttempts $\leftarrow$ 0
      \While{$\neg$ \success and \nrAttempts $<$ THRESHOLD}
        \State $\nrAttempts \leftarrow \nrAttempts + 1$
        \State $t'' \leftarrow$ extend $t'$ at $E$ with code suggested by LLM
        \If{$t''$ not syntactically valid or $t'' \in \TAttempted$}
          \State \textbf{continue}
        \EndIf 
        \State $\feedback \leftarrow$ $\execute{$t''$}$
        \If{\feedback shows successful execution}
          \State $\TAssert \leftarrow \TAssert \cup \{ t'' \}$
          \State $t''' \leftarrow \addExtensionPoints{$t''$}$
          \State $W \leftarrow W \cup \{ t''' \}$
          \State $\success \leftarrow true$
        \ElsIf {\feedback shows assertion failure}
          \State $t''' \leftarrow$ comment out assertions in $t''$
          \State $\TNoAssert \leftarrow \TNoAssert \cup \{ t''' \}$ \Comment{note: not setting success to true, not adding this test to W}
        \Else \Comment{if feedback shows that a runtime error happened}
          \State $\TFail \leftarrow \TFail \cup \{ t'' \}$
        \EndIf
      \EndWhile   
    \EndWhile

    \State \Return{$\langle$ \TAssert, \TNoAssert, \TFail $\rangle$}
\end{algorithmic}
\end{algorithm}


==> figures/alg-docsnippetmining.tex <==
\begin{algorithm}[tb]
\caption{Pseudo-code for mining snippets from documentation.}
\label{alg:SnippetMiningFromDocs}
{\footnotesize
\begin{algorithmic}[1]
	\Function{\textit{getSnippets}}{\pkgName, \sigs}
	
    \State $H$ $\leftarrow$ map that maps each \sig in \sigs to $\emptyset$ \label{line:initializeMap} \Comment{initialize map} \label{line:DocSnippetMiningInitializeMap}
	\\ 
	\State \snippets $\leftarrow$ $\emptyset$  \Comment{gather all snippets} \label{line:GatherSnippetsStart}
	\For{each markdown file $f$ in the repository of \pkgName}
	  \For{each fenced code block $b$ in $f$}
	     \State \Comment{assume a new snippet starts when a variable is redeclared} 
	     \For{each \snippet in $b$} 
	       \State \snippets $\leftarrow$ \snippets $\cup$ \snippet
	     \EndFor
	  \EndFor
	\EndFor \label{line:GatherSnippetsEnd}
 
    \\   
	\For{each \snippet in \snippets}  \Comment{associate snippets with signatures} \label{line:AssociateSnippetsWithSigsStart}
	  \For{each \sig in \sigs}
	    \If{\sig occurs in \snippet}
	      \State $H(\sig) \leftarrow H(\sig) \cup \snippet$  
	    \EndIf
	  \EndFor
	\EndFor  \label{line:AssociateSnippetsWithSigsEnd}
	  
	\\ 
	
    \For{each \sig in \sigs}  \Comment{\begin{tabular}[t]{r} select dissimilar examples\\for each signature\end{tabular}} \label{line:SelectDissimilarSnippetsStart}
      \State \snippets $\leftarrow H(\sig)$
	  \State \partitions $\leftarrow$ \{ \{ $s$ \} $|$ $s \in \snippets$ \} \label{line:CreatePartitions} \Comment{create partitions}
      \While{$|\partitions|$ $>$ MAX\_SNIPPETS} \label{line:LoopMergePartitionsStart}
        \State \Comment{\begin{tabular}[t]{r}merge the partitions that are most similar\end{tabular}}
        \State find partitions $p_1,p_2$ such that: \label{line:MergePartitionsStart} \\
		     \hspace*{1.5cm}$\forall p,p' \in \partitions$: \similarity{p_1}{p_2} $\leq$ \similarity{p}{p'}
        \State \partitions = \partitions $-$ $p_1$ $-$ $p_2$ $+$ $(p_1 \cup p_2)$ \label{line:MergePartitionsEnd}
      \EndWhile \label{line:LoopMergePartitionsEnd}
      \\
      \State \Comment{select the smallest snippet from each partition}
      \State \snippets $\leftarrow$ \{ \begin{tabular}[t]{l} \label{line:SelectSmallestSnippetStart}
        $s$ $|$ $s \in p$, $p \in \partitions$,\\
	    $\forall s' \in p$: $\length{s} \leq \length{s'}$  \} 
	  \end{tabular} \label{line:SelectSmallestSnippetEnd}
	 \State $H(\sig)$ $\leftarrow$ \snippets \label{line:updateMap}
   \EndFor \label{line:SelectDissimilarSnippetsEnd}	 
		   
    \\
    \State {\bf return} $H$  \label{line:returnMap}
	\EndFunction
\end{algorithmic}
}
\end{algorithm}


==> overview.tex <==
\section{Background and Overview}

From a user's perspective, a \emph{generative language model} is very simple:
given a piece of text (known as the \emph{prompt}), the model predicts how the
text continues. Large language models like OpenAI's Codex model~\cite{codex21}
have been trained on both natural language and source code, and hence the text
can be either natural language or code, making them immediately useful for tasks
like smart completion in an IDE as shown by tools like GitHub Copilot and Amazon
Code Whisperer.

This is quite natural, since during training the models are trained on exactly
this kind of task.

It is less clear that such models can also be used for other tasks beyond code
completion, but any frequent user of a generative language model will soon
observe that the models generalize surprisingly well in practice, given
appropriate descriptions of the task embedded into the prompt. It is also easy
to observe that careful prompt design is crucial, all the more so since current
language models have a fairly limited prompt size (measured in kilobytes),
making it infeasible to, e.g., put an entire code base into the prompt.

\begin{figure*}
\includegraphics[width=\textwidth]{figures/new-diagram-V2.pdf}
\caption{Overview of \toolname}
\label{fig:overview}
\end{figure*}

Based on this general observation, we choose to focus on two pieces of data to
embed into the prompt:

\begin{enumerate}
\item The signature of the function to test, including the name of the function
itself and its arguments. Due to the dynamic typing discipline of JavaScript,
the signature does \emph{not} include parameter or return types.
\item A list of code snippets containing calls the function to test.
\end{enumerate}

Note, in particular, that we do \emph{not} include the implementation of the
function itself in the prompt, since it could be arbitrarily long and hence
overrun the maximum prompt size. Thus we end up with a ``black box'' model,
whereby the model only gets information about the function as seen from a user's
perspective.

At a high level, the overall system functions as shown in
Figure~\ref{fig:overview}: starting from an npm package to generate tests for,
the \emph{API explorer} extracts the signatures of all public API functions,
while the \emph{snippet miner} extracts example usage snippets. API exploration
is done dynamically by loading the package and reflectively exploring the object
graph it exports. Snippet mining, on the other hand, is implemented as a simple
static analysis in CodeQL, combining an approximate call-graph builder with a
lightweight intra-procedural backwards-slicing algorithm.

For each function signature and associated snippets, the \emph{test generator}
iteratively generates tests following the feedback-directed random test
generation paradigm: starting from a simple stub instructing the model to
generate a call to the function under test, we repeatedly extend the partial
test by guiding the model towards generating calls for other functions. At each
step, a prompt including the function signature, example snippets, and partial
test generated so far is packaged into a prompt and sent to the model for
completion.

Once we have generated the desired number of candidate tests, the \emph{test
validator} filters out tests that are invalid or do not pass, leaving us with a
final set of generated tests.

==> testgeneration.tex <==
\section{Approach}

This section presents the key steps of our approach:
  (i)   API exploration,
  (ii)  snippet mining, and
  (iii) test generation.

\input{figures/alg-APIexploration}
  
\subsection{API Exploration}

This step takes a package under test, \pkgName, and produces a list of pairs $\Pair{a}{t}$ representing its API.
Here, $a$ is an \textit{access path} that uniquely represents an API method, and $t$ is a description of that method's type.
Our notion of an access path takes a somewhat simplified form compared to the original concept proposed by
Mezzetti et al. \cite{mezzetti18}, and consists of a package name followed by a sequence of property names, and
a \textit{type descriptor} consists of a method signature, or one of the string values ``array'', ``number'', ``string'',
``object'', or ``boolean''.        

We rely on a dynamic approach to explore the API of a package \pkgName, which is outlined in Algorithm\ref{alg:exploreAPI}.  
This is accomplished by creating a small program that imports the package (line~\ref{line:createModObj}), and relying on 
JavaScript's introspective capabilities to determine which properties are present in the \textit{package root} object \modObj 
that is created by importing \pkgName and what types these properties have. 
Exploration of  \modObj's properties is handled by a recursive function is handled by an auxiliary function \textit{explore} , which  
traverses this object recursively, calling another auxiliary function \textit{extend} to extend the access path as the traversal 
descends into the object's structure.   

During exploration, if a property $p$ is discovered at access path $a$  whose type is a function $f(\cdots)$, then an 
pair $\Pair{a}{f(\cdots)$} is recorded (line~\ref{line:RecordFunctionProperty}). If the type of $p$ is an array,
then the array's elements are recursively explored (line~\ref{line:ExploreArrayElementsStart}--\ref{line:ExploreArrayElementsEnd}), 
and if the type of $p$ is an object, then $p$'s properties are explored recursively as well (line~\ref{line:ExploreObjectPropsStart}).
\TODO{why do we not assign the type descriptor in the object case?}    


\subsection{Snippet Mining}

Our approach gathers usage examples (henceforth referred to as ``snippets'') from a project's documentation that illustrate how a given 
API method is to  be used. These examples are incorporated into the prompt that is sent to the LLM. We now present some details of this technique.



  
\input{figures/alg-docsnippetmining}   
   
 
Figure~\ref{alg:SnippetMiningFromDocs} shows pseudo-code for mining usage examples from documentation. The figure shows
a function \code{getSnippets} that takes two arguments: the name \pkgName of a package, and a set \sigs of signatures of API methods
for which examples should be found. Function \code{getSnippets} returns a map from signatures to sets of usage examples.  

Line~\ref{line:DocSnippetMiningInitializeMap} initializes a map $H$ by associating an empty set of snippets with each signature in \sigs.
Next, lines~\ref{line:GatherSnippetsStart}--\ref{line:GatherSnippetsEnd} gather the snippets by finding each fenced code block within
each markdown file in the distribution of \pkgName. We found that a single fenced code block sometimes contains multiple distinct examples;
to handle such cases, we assume that a new example starts when a redeclaration is seen for a variable that was declared previously in the same
code block%
\footnote{
  In our implementation, this is handled by using regular expression matching to determine when variables are being declared and keeping
  track of a set of previously declared variables. For details, the reader is referred to our code artifact \TODO{need to submit an artifact}.   
}.  

On lines~\ref{line:AssociateSnippetsWithSigsStart}--\ref{line:AssociateSnippetsWithSigsEnd}, code snippets are associated with signatures.
Concretely, a signature \sig = $m(v_1,\cdots,v_n)$ is associated with every snippet in which the method name $m$ occurs textually.  

In practice, we found that documentation may contain many examples that are highly similar and repetitive. Since the amount of space
available for including snippets in a prompt is limited, our approach aims to select a subset of the set of snippets that are
dissimilar to each other, by executing the loop of lines~\ref{line:SelectDissimilarSnippetsStart}--\ref{line:SelectDissimilarSnippetsEnd}
for each signature \sig.  

To this end, the algorithm employs a clustering approach that involves creating a set of partitions and repeatedly merging
the two partitions containing the snippets that are the most similar to each other.  Initially, each snippet is in a partition containing
just itself (line~\ref{line:CreatePartitions}). Then, as long as more than MAX\_SNIPPETS partitions exist, the loop on 
lines~\ref{line:LoopMergePartitionsStart}--\ref{line:LoopMergePartitionsEnd} is executed.
Each iteration of the loop involves using Definition~\ref{def:similarity} to find the two partitions $p_1$ and $p_2$ that are the most similar 
to each other and merging them (lines~\ref{line:MergePartitionsStart}--\ref{line:MergePartitionsEnd}). 
When exactly MAX\_SNIPPETS partitions are left, the algorithm selects the smallest snippet from each partition
(lines~\ref{line:SelectSmallestSnippetStart}--\ref{line:SelectSmallestSnippetEnd}) and updates the map $H$ (line~\ref{line:updateMap}).  

Finally, when all signatures have been processed, the map $H$ is returned (line~\ref{line:returnMap}).  

\begin{definition}[similarity] \label{def:similarity}
  Let $S_1$ and $S_2$ be sets of strings. Define:
  \[
    \similarity{S_1}{S_2} = \Min{ \{ \Levenshtein{s_1}{s_2}  | s_1 \in S_1,\: s_2 \in S_2 \} } 
  \]
  where \textit{Levenshtein} computes the Levenshtein edit distance between two strings. \TODO{do we need a citation for Levenshtein distance?}
\end{definition} 

\input{figures/alg-testgeneration}

\TODO{are there any implementation details that we need to discuss here? E.g., adding import statements, etc.?}

\subsection{Test Generation}

Algoritm~\ref{alg:TestGeneration} shows pseudo-code for our test generation algorithm as a function \textit{generateTests}.
This function takes as a parameters the name \pkgName of a package for which tests should be generated and a bound $N$ on
the number of tests that should be generated and it returns sets
   \TAssert, \TNoAssert, and \TFail
representing 
   passing tests with assertions,
   passing tests without assertions, and
  failing tests, respectively.

We briefly discuss the workings of the algorithm. On line~\ref{line:callExploreAPI}, Algorithm~\ref{alg:exploreAPI} is applied
to explore the package's API, resulting in a set of signatures \sigs. On line~\ref{line:callGetSnippets}, Algorithm~\ref{alg:SnippetMiningFromCode}
is applied to find examples for the signatures in \sigs, resulting in a map $H$ that maps each signature to a set of examples.   
Line~\ref{line:createInitialTest} creates (the prefix for) an initial test $t_{\mbox{\scriptsize \it init}}$, consisting of a test harness into which specific tests can be added.
\TODO{include some Mocha scaffolding code into this, with describe/it functions}.
Line~\ref{line:initializeWorklist} initializes a worklist $W$ to include $t_{\mbox{\scriptsize \it init}}$, and
line~\ref{line:initializeAttempted} initializes a set $\TAttempted$ of tests that have been attempted, which is used to avoid duplicate work.

On line~\ref{line:beginTestGenerationLoop}, the algorithm enters a loop in which tests are generated repeatedly until $N$ tests have been created.
\TODO{should be bound be based on a time budget instead, or on the number of successful tests that have been generated?}
In each iteration of the loop, the algorithm:
  selects a test $t$ from $W$ (line~\ref{line:selectTestFromWorklist}),
  selects an extension point $E$ in this test (line~\ref{line:selectExtensionPoint}),
  selects a signature \sig from \sigs (line~\ref{line:selectSignature}),
  retrieves  usage examples $h$ for $s$ from $H$ (line~\ref{line:getSnippetsForSig}),
  extends $t$ at $E$ with a comment indicating that code for testing \sig should be added there (line~\ref{line:addPromptToTest}),
  and extends the resulting test $t'$ with the usage examples $h$ (line~\ref{line:addSnippetsToTest}).
    
The algorithm's inner loop (lines~\ref{line:InnerLoopStart}--\ref{line:InnerLoopEnd}) then repeatedly tries suggestions
offered by the LLM. To this end,  $t'$ is extended with code fragments suggested by the LLM (line~\ref{line:ApplyLLMSuggestion}).
If the resulting test $t''$ is syntactically correct (line~\ref{line:checkSyntacticValidity}) and has not been tried before
(line~\ref{line:checkSyntacticValidity}), it is executed (line~\ref{line:executeTest}) resulting in execution \feedback
that reflects whether the execution terminated normally, if a crash occurred, or if some assertion failure occurred.
If execution was successful, $t''$ is added to \TAssert (line~\ref{line:AddToTAssert}), extension points in this new test
are identified (line~\ref{line:AddExtensionPoints}), and the resulting test is added to $W$ (line~\ref{line:AddToWorkList}).
In the case of assertion failures, the failed assertions are commented out (line~\ref{line:CommentOutFailingAssertions}) 
and the resulting test is added to \TNoAssert (line~\ref{line:AddToTNoAssert}).
In the case of a crash, the resulting test is added to \TFail (line\ref{line:AddToTFail}).  



